Deep Analysis on Subgraph Isomorphism

Subgraph isomorphism is a well-known NP-hard problem which is widely used in many applications, such as social network analysis and knowledge graph query. Its performance is often limited by the inherent hardness. Several insightful works have been done since 2012, mainly optimizing pruning rules and matching orders to accelerate enumerating all isomorphic subgraphs. Nevertheless, their correctness and performance are not well studied. First, different languages are used in implementation with different compilation flags. Second, experiments are not done on the same platform and the same datasets. Third, some ideas of different works are even complementary. Last but not least, there exist errors when applying some algorithms. In this paper, we address these problems by re-implementing seven representative subgraph isomorphism algorithms as well as their improved versions, and conducting comprehensive experiments on various graphs. The results show pros and cons of state-of-the-art solutions and explore new approaches to optimization.

==> graphql.tex <==

\subsection{GQL Algorithm} \label{sec:graphql}
GQL addresses the problem by combination of techniques: use of neighborhood subgraphs and profiles, joint reduction of the search space and optimization of the search order. Finally, GQL performs DFS to get all matches.

GQL firstly reduces the candidate set of each nodes by use of the local information i.e. neighborhood subgraphs or neighborhood profile.
\begin{definition}\label{def:nei_subgraph} \textbf{(Neighborhood Subgraph)}
	Given graph $G$, node $v$ and radius $r$, the neighborhood subgraph of node v consists of all nodes within distance $r$ (number of hops) from $v$ and all edges between nodes.
\end{definition}
\begin{definition}\label{def:nei_profile} \textbf{(Neighborhood Profile)}
	Given graph $G$, node $v$ and radius $r$, the neighborhood profile of node v is a set of node labels within distance $r$ (number of hops) from $v$ and all edges between nodes.
\end{definition}

Although neighborhood subgraphs have high pruning power because of graph structures, the time and space complexity can be relatively high. Neighborhood profile can prune candate set in linear time despite of less pruning power. We choose neighborhood profile to implement the algorithm.

\begin{definition}\label{def:semi_perfect} \textbf{(Semi-perfect matching $B(u,v)$)}
	For each neighbor $d$ of $u$, if there is a neighbor $g$ of $v$ s.t. $g\in C(u)$, then B(u,v) is a semi-perfect matching.
\end{definition}

Then, we perform joint reduction by adjacent edges of vertices. For each candidate data vertex $v$ of a query vertex $u$, we construct bipartite graph $B(u,v)$. If for each neighbor $u'$ of $u$ there is a neighbor $v'$ of $v$ in the candidate set of $u'$, the bipartite graph $B(u,v)$ is semi-perfect match. When $B(u,v)$ is not semi-perfect match, it means $v$ cannot be a candidate of $u$ and we remove $v$ from $C(u)$. 

To avoid unnecessary and endless joins, a pair $(u,v)$ is $marked$ if it needs to be checked for semi-perfect matching where $u$ is a query vertex and $v$ is a data vertex. When $B(u,v)$ is a semi-perfect match, then $unmark$ $(u,v)$. When $B(u,v)$ is not semi-perfect match, it means neighbors of this query vertex may have smaller candidate set. So we mark its neighbors' query vertices and candidates pair to check the semi-perfect matches of them. Joint reduction finishes when there is no marked $(u,v)$.
%\begin{figure}[htbp]   
%	\centering
%	\includegraphics[width=8cm]{\picfolder graphql.pdf}   
%	\vspace{-0.1in}          
%	\caption{Filtering of GraphQL}        
%	\label{fig:graphql}   
%\end{figure}
\begin{table}[htbp] 
	\caption{Filtering of GQL} 
%	\resizebox{\textwidth}{12mm}
%	\resizebox{\linewidth}{!}{\rule{1.1\linewidth}{3cm}}
	\label{table:graphql}
	\centering
	\begin{tabular}{|p{7mm}|p{20mm}|p{20mm}|p{20mm}|}  
		\hline
%		\cline{2-3}
		& before filtering & 1-hop neighbor profile & semi-perfect match  \\
		\hline
		$C(u_{0})$ &$v_{0},v_{203}$&$v_{0},v_{203}$ &$v_{0},v_{203}$ \\
		\hline
		$C(u_{1})$ &$v_{1},v_{2},...,v_{99}$&$v_{1},v_{2},...,v_{99}$ &$v_{1}$ \\
		\hline
		$C(u_{2})$ &$v_{101},v_{102},...,v_{202}$&$v_{101},v_{202}$ &$v_{101}$ \\
		\hline	
		$C(u_{3})$ &$v_{101},v_{102},...,v_{202}$&$v_{101},v_{102},...,v_{202}$ &$v_{101},v_{102}$ \\
		\hline
		$C(u_{4})$ &$v_{101},v_{102},...,v_{202}$&$v_{101},v_{102},...,v_{202}$ &$v_{101},v_{102}$ \\
		\hline
	\end{tabular}
\end{table}

For example in Table \ref{table:graphql}, we perform GQL with simplest settings on Figure \ref{fig:example}. When filtering based on 1-hop neighbor, candidates of $u_{2}$ are significantly reduced to 2 vertices because other candidates do not have neighbor with label $B$. Assume that we perform joint reduction with the order $u_{0}$ to $u_{4}$ that actually simplifies the $mark$ and $unmark$ procedure. Candidate set of $u_{1}$ is reduced to only one vertex because other candidates are not adjacent to $v_{201}$ or $v_{202}$ while $u_{1}'s$ neighbor $u_{2}$ have candidates set $\{v_{201},v_{202}\}$. Similarly, candidate sets of $u_{3}, u_{4}$ are also significantly reduced.




%If the semi-perfect matching $B(u,v)$ exists, the pair $<u,v>$ is unmarked. If $B(u,v)$ does't exist, it means candidates of neighbors of $u$ are more likely to be pruned. Therefore, mark $<u',v'>$ for each $u^{\prime} \in N_{\mathcal{P}}(u), v^{\prime} \in N_{G}(v), v^{\prime} \in \Phi\left(u^{\prime}\right)$. When all $<query_vertex, data_vertex>$ pairs are unmarked, joint reduction step finishes.

A search order can be represented as a rooted binary tree whose leaves are nodes of the graph pattern and each internal node is a join operation. To optimize the search order, GQL proposes a cost model of join operation.
%\begin{definition}\label{def:res_size_of_join} \textbf{(Result size of join)}
%	The result size of join(edge) $i$ s estimated by 
%	$$
%	\text { Size }(i)=\text { Size }(i . l e f t) \times \text { Size }(i . r i g h t) \times \gamma(i)
%	$$
%	where $i.left$ and $i.right$ are the left and right child nodes of $i$ respectively, and $\gamma(i)$ is the reduction factor.
%\end{definition}
%$$
%\gamma(i)=\prod_{e(u, v) \in \mathcal{E}(i)} P(e(u, v))
%$$
%$$
%P(e(u, v))=\frac{f r e q(e(u, v))}{f r e q(u) \cdot f r e q(v)}
%$$
\begin{definition}\label{def:cost_of_join} \textbf{(Cost of join)}
	The cost of join $i$ s estimated by 
	$$
	\operatorname{cost}(i)=\operatorname{Size}(i . l e f t) \times \text { Size (i.right) }
	$$
\end{definition}
The total cost of search order $\Gamma$ is estimated by 
$$
\operatorname{cost}(\Gamma)=\sum_{i \in \Gamma} \operatorname{cost}(i)
$$

Based on this cost model, we can choose best order to perform dfs.



==> quicksi.tex <==

\subsection{QSI Algorithm} \label{sec:quicksi}

QSI solves subgraph containment query problem and we adjust it to solve subgraph isomorphism problem. It uses QI-sequence to encode a search order and topological information of the query graph. It also decides a QI-sequence order based on the weighted query graph to bound the search space.


QI-Sequence represents a rooted spanning tree for the query graph. It consisits of a list of $spanning entries$,$T_{i}$, for $1 \leq i \leq |V|$  Other edges outside of the spanning tree are added as $extra entries$. A QI-Sequence of $q$ is $SEQ_{q}=\left[\left[T_{i} R_{i j}^{*}\right]^{\beta}\right]$. $T_{i}.v$ records a vertex index. $T_{i} \cdot p$ stores the parent QI-Sequence entry id of $T_{i}.v$ in the spanning tree and $T_{i}.l$ stores the label of $T_{i}.v$. The subindex $i$ of $T_{i}$ specifies the search order. $R_{ij}$ is extra entries about $T_{i}$. It stores degrees and edges outside of the spanning tree. There are two kinds of extra entries in $R_{ij}$, namely $degree constraint$ and $extra edge$. The $degree constraint$ is $[deg:d]$ where $d$ is the degree of $v_{i}$. The $extra edge$ in $R_{i j}$ is $[edge:j]$, which means there is an extra edge between $T_{i}.v$ and $T_{j}.v$ for $j<i$.

After query graph is converted into a QI-Sequence, we use dfs algorithm to search subgraph isomorphism in the data graph. We select a candidates set at depth $d$ which satisfies the label and edge in the spanning tree of SEQ. Then we filter this candidates set using $R_{ij}$ to meet degree constraint and extra edges. After choose a valid candidate, the algorithm goes to $d+1$ step and then backtrack.

\begin{definition}\label{def:search_breadth} \textbf{(Search Breadth)}
	The search breadth 
	$$
	B_{i}=|\left\{ {H}^{i} | {H}^{i}:SEQ_{q}^{i} \rightarrow g\right\} | (1 \leq i \leq |V|)\}
	$$
	where $S E Q_{q}^{i}=\left[\left[T_{i} R_{i j}^{*}\right]^{i}\right]$ is a prefix of $S E Q_{q}$
\end{definition}

Given the QI-Sequence with length $i$ and the data graph $g$, the search breadth is matchings of QI-Sequece in data graph.

We need to generate an effective QI-Sequence $S E Q_{q}$ as the best search order to bound the search breadth.

\begin{definition}\label{def:inner_support} \textbf{(Inner support)}
Given a query graph $q$ and a data graph $g$, the inner support $\phi(q, g)$ is the number of isomorphic mappings from $q$ to $g$.
\end{definition}

It is immediate that the search breadth $B_{i}$ is $\phi\left(S E Q_{q}^{i}, g\right)$

We count inner support of vertices and edges, i.e. 1-vertex and 1-edge features only considering labels.
$$
\phi_{a v g}(v)=|\{f | f(v) \in V(g) \}|
$$

$$
\phi_{a v g}(e)=|\{f | f(v) \in V(g) \}|
$$

Then we add these inner supports as weights to the vertices and edges of the query graph $q$ and convert $q$ to a weighted graph $q^{w}$. Then we find the minimum spanning tree of $q$ based on the edge weights.

To begin with, we select the edge with the least weight as the first edge and choose the vertex with lower weight in the first edge as the first vertex. Then we expand the spanning tree choosing the edge which makes the induce subgraph of current vertex set as dense as possible. If there are more than one candidates, we then select edges whose endpoint has the least degree. Finally, we randomly select edges from edges with least weight in the candidate set. For other newly added adjacent edges which are not in the spanning tree, we sort them by the increasing order of $w(e)$ and store them as $extra edge$ items.

\begin{figure}[htbp]   
	\centering
	\includegraphics[width=8cm]{\picfolder quicksi.pdf}   
	\vspace{-0.1in}          
	\caption{Exampel of QSI}        
	\label{fig:quicksi}   
\end{figure}

Figure \ref{fig:quicksi} shows the structure of QSI corresponding to Figure \ref{fig:example}. We choose $(u_{0}, u_{2})$ as the first edge because of least edge weight and choose $u_{0}$ as the first vertex because of the lower vertex weight. Then we choose $(u_{0}, u{1})$ as next tree edge because its edge weight is lower than $(u_{2}, u{1})$.  


